Transferring Fairness under Distribution Shifts via Fair Consistency Regularization

The increasing reliance on ML models in high-stakes tasks has raised a major concern on fairness violations. Although there has been a surge of work that improves algorithmic fairness, most of them are under the assumption of an identical training and test distribution. In many real-world applications, however, such an assumption is often violated as previously trained fair models are often deployed in a different environment, and the fairness of such models has been observed to collapse. In this paper, we study how to transfer model fairness under distribution shifts, a widespread issue in practice. We conduct a fine-grained analysis of how the fair model is affected under different types of distribution shifts and find that domain shifts are more challenging than subpopulation shifts. Inspired by the success of self-training in transferring accuracy under domain shifts, we derive a sufficient condition for transferring group fairness. Guided by it, we propose a practical algorithm with a fair consistency regularization as the key component. A synthetic dataset benchmark, which covers all types of distribution shifts, is deployed for experimental verification of the theoretical findings. Experiments on synthetic and real datasets including image and tabular data demonstrate that our approach effectively transfers fairness and accuracy under various distribution shifts.

==> tables/ablation.tex <==


\begin{figure}[!htbp]
\centering
    \begin{subfigure}[c]{0.4\textwidth}
        \begin{center}
        \includegraphics[width=\textwidth]{figs/ablation.png}
        \caption{\textbf{Figure~\ref{fig:fcr}}:Group accuracy and consistency evaluated on the target data. Accuracy is correlated with consistency. Comparing with the standard consistency regularization (SCR), the model trained with fair consistency regularization (FCR) has more balanced consistency and accuracy.}\label{fig:fcr}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.58\textwidth}
        \begin{center}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{llll}
        \toprule
                      &        Acc & \multicolumn{2}{c}{Unfairness}\\
               \cline{3-4}
        Method         &   & $V_{acc}$  & $\Delta_{odds}$ \\
        \midrule
        Ours & \facc{84.65}{1.13} & \facc{2.92}{0.72} & \facc{6.99}{0.41}   \\
        w/o consistency in target & \facc{81.60}{0.45} &  \facc{10.01}{1.59}  & \facc{4.17}{0.39}  \\
        w/o consistency in source & \facc{83.49}{0.61} &  \facc{6.76}{0.82}  & \facc{5.68}{1.24}  \\
        w/o dynamic weights & \facc{84.87}{1.69} &  \facc{4.05}{2.06}  & \facc{7.18}{1.93}  \\
        w/o updating $g_{tc}$ & \facc{79.11}{0.46} &  \facc{2.45}{0.13}  & \facc{7.19}{2.20}  \\
        \bottomrule
        \end{tabular}
        }
        \end{center}
        \caption{\textbf{Figure~\ref{tab:ablation}}: Model's performance in the target domain. \fhc{caption}.}\label{tab:ablation}
    \end{subfigure}
    \vspace{-1em}
    %\caption{    }
\end{figure}


% \begin{table}[!htbp]
% \small
% \centering
% \caption{Model's performance in the target domain} 
% \begin{tabular}{llll}
% \toprule
%                       &        Acc & \multicolumn{2}{c}{Unfairness}\\
%               \cline{3-4}
% Method         &   & $V_{acc}$  & $\Delta_{odds}$ \\
% \midrule
% Ours (Laftr+FairFixMatch) & \facc{84.65}{1.13} & \facc{2.92}{0.72} & \facc{6.99}{0.41}   \\
% w/o consistency in target & \facc{81.60}{0.45} &  \facc{10.01}{1.59}  & \facc{4.17}{0.39}  \\
% w/o consistency in source & \facc{83.49}{0.61} &  \facc{6.76}{0.82}  & \facc{5.68}{1.24}  \\
% w/o dynamic weights & \facc{84.87}{1.69} &  \facc{4.05}{2.06}  & \facc{7.18}{1.93}  \\
% w/o updating $g_{tc}$ & \facc{79.11}{0.46} &  \facc{2.45}{0.13}  & \facc{7.19}{2.20}  \\



% \bottomrule
% \end{tabular}
% \label{tab:ablation}

% \end{table}

==> tables/app-resnet.tex <==
\begin{table}[!htbp]
\captionsetup{font=footnotesize}
\small
\centering
\vspace{-0.5em}
\caption{Transfer fairness and accuracy from UTKFace to FairFace with ResNet18} 
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{llllllll}
\toprule
               & \multicolumn{3}{c}{Source}            && \multicolumn{3}{c}{Target}            \\ 
               \cline{2-4} \cline{6-8} 
                              & Acc  & \multicolumn{2}{c}{Unfairness} && Acc & \multicolumn{2}{c}{Unfairness}\\
               \cline{3-4} \cline{7-8}
Method         &    & $V_{acc}$ & $\Delta_{odds}$ &  & & $V_{acc}$ & $\Delta_{odds}$ \\
\midrule
Base           & \facc{90.12}{0.75} &  \facc{1.79}{0.33}  & \facc{4.83}{1.83} && \facc{71.47}{0.86} & \facc{11.88}{3.24} & \facc{4.07}{1.05}   \\
Laftr           & \facc{90.20}{0.09} &  \facc{1.91}{0.69}  & \facc{4.55}{0.81} && \facc{70.97}{0.44} & \facc{14.39}{4.49} & \facc{4.35}{2.76}   \\
CFair          & \facc{89.72}{0.42} &  \facc{1.84}{0.59}  & \facc{4.13}{2.11} && \facc{70.67}{1.08} & \facc{15.29}{3.54} & \facc{4.29}{1.34}   \\
\midrule
Laftr+DANN      & \facc{89.55}{0.72} &  \facc{3.10}{1.95}  & \facc{5.46}{1.31} && \facc{70.95}{0.90} & \facc{4.04}{2.04} & \facc{5.75}{1.64}   \\
Laftr+MMD      & \facc{89.34}{0.70} &  \facc{3.11}{0.48}  & \facc{6.77}{1.51} && \facc{69.50}{0.66} & \facc{5.59}{1.49} & \facc{8.32}{1.85}   \\
% Laftr+FixMatch & 95.64 & 1.33 & 2.00 & 4.18 && 84.54 & 10.3 & 3.86 & 3.85    \\
% Ours (Laftr+FairFixMatch) &94.66 & 0.59 & 0.95 & 1.78 && 86.12 & 1.87 & 3.66 & 7.41  \\
Laftr+FixMatch  & \facc{95.22}{0.44} &  \facc{1.72}{0.42}  & \facc{3.54}{0.96} && \facc{83.97}{0.42} & \facc{9.26}{0.82} & \facc{5.03}{0.52}   \\
CFair+FixMatch  & \facc{94.97}{0.54} &  \facc{1.39}{0.79}  & \facc{2.63}{1.05} && \facc{82.99}{0.75} & \facc{11.43}{0.73} & \facc{4.33}{0.72}   \\
% Laftr+UDA& \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}   \\
Ours (w/ Laftr)  & \facc{94.56}{0.94} &  \facc{2.29}{1.21}  & \facc{1.74}{1.02} && \facc{84.10}{0.95} & \facc{5.90}{2.07} & \facc{7.95}{0.77}   \\
% Ours (Laftr+FairUDA)  & \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}  \\
Ours (w/ CFair)  & \facc{94.99}{0.25} &  \facc{1.39}{0.31}  & \facc{2.17}{0.60} && \facc{84.31}{0.67} & \facc{7.43}{1.67} & \facc{6.77}{1.55}   \\
\bottomrule
\end{tabular}\label{tab:face-resnet_rand}
}
\end{table}

==> tables/dataset.tex <==

\begin{table}[h]
\small
\begin{tabular}{cccccc}
\toprule
\multicolumn{2}{c}{$(Y, A)$}            & (Male, White) & (Male, Non-white) & (Female, White) & (Female, Non-white) \\ 
\midrule
\multirow{2}{*}{UTK (S)}      & train &   1373            &   750                & 1650                &     1227                \\ \cmidrule{2-6} 
                              & test  &    565         &   285               &   614            &      370              \\ 
                              \midrule
\multirow{2}{*}{FairFace (T)} & train &     11429            &   16574                   &      8024            &   16838                      \\ \cmidrule{2-6} 
                              & test  &    1712           & 2453                  &   1176              &     2518                \\ 
                             \bottomrule
\caption{Statistics of UTK and FairFace datasets.}
\label{tab:dataset_face}
\end{tabular}
\end{table}

\begin{table}[h]
\small
\begin{tabular}{cccccc}
\toprule
\multicolumn{2}{c}{$(Y, A)$}            & (High, Male) & (High, Female) & (Low, Male) & (Low, Female) \\ 
\midrule
\multirow{2}{*}{CA (S)}      & train &      33258         &       22314            &     39224            &    42169                 \\ \cmidrule{2-6} 
                              & test  &   14839            &    9924           &    15990             &      17947                \\ 
                              \midrule
\multirow{2}{*}{Other states (T)} & train &  232162             &        140876           &      296826           &      351970               \\ \cmidrule{2-6} 
                              & test  &   101934           &      57798             &   127654              &   150544                  \\ 
                             \bottomrule
\caption{Statistics of NewAdult dataset.}
\label{tab:dataset_newadult}
\end{tabular}
\end{table}

==> tables/utk-fairface-weak.tex <==
% \begin{table}[ht]
% \small
% \centering
% \caption{Transfer fairness and accuracy from UTKFace to FairFace with weak transformations} 
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{llllllllll}
% \toprule
%               & \multicolumn{4}{c}{Source}            && \multicolumn{4}{c}{Target}            \\ 
%               \cline{2-5} \cline{7-10} 
%                               & Acc  & \multicolumn{3}{c}{Unfairness} && Acc & \multicolumn{3}{c}{Unfairness}\\
%               \cline{3-5} \cline{8-10}
% Method         &    & $V_{acc}$ & $\Delta_{acc}$ & $\Delta_{odds}$ &&   & $V_{acc}$ & $\Delta_{acc}$ & $\Delta_{odds}$ \\
% \midrule

% Laftr+FixMatch & \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0}  \\
% Laftr+UDA& \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0}  \\
% Ours (Laftr+FairFixMatch) & \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0}  \\
% Ours (Laftr+FairUDA)  & \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0}  \\
% Ours (CFair+FairFixMatch) & \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0}  \\
% \bottomrule
% \end{tabular}\label{tab:face-vgg_weak}
% }
% \end{table}

\begin{table}[]
\small
\centering
\caption{Transfer fairness and accuracy from UTKFace to FairFace with weak transformations} 

\begin{tabular}{llllllll}
\toprule
               & \multicolumn{3}{c}{Source}            && \multicolumn{3}{c}{Target}            \\ 
               \cline{2-4} \cline{6-8} 
                              & Acc  & \multicolumn{2}{c}{Unfairness} && Acc & \multicolumn{2}{c}{Unfairness}\\
               \cline{3-4} \cline{7-8}
Method         &    & $V_{acc}$ & $\Delta_{odds}$ &  & & $V_{acc}$ & $\Delta_{odds}$ \\
\midrule
Laftr+FixMatch  & \facc{92.29}{0.32} &  \facc{1.09}{0.42}  & \facc{4.27}{1.09} && \facc{76.38}{0.42} & \facc{16.64}{2.86} & \facc{6.21}{1.52}   \\
% Laftr+UDA& \facc{0.0}{0.0} &  \facc{0.0}{0.0}  & \facc{0.0}{0.0} & \facc{0.0}{0.0} && \facc{0.0}{0.0} & \facc{0.0}{0.0}   \\
Ours (Laftr+FairFixMatch)  & \facc{92.82}{0.41} &  \facc{1.46}{0.85}  & \facc{4.88}{1.56} && \facc{77.13}{0.92} & \facc{4.68}{0.90} & \facc{6.98}{0.51}   \\
\bottomrule
\end{tabular}\label{tab:face-vgg_weak}
\end{table}

% \begin{table}[ht]
% \centering
% \caption{Transfer fairness and accuracy from UTKFace to FairFace with VGG16 (Crop+Flip)}
% \begin{tabular}{llllllllll}
% \toprule
%               & \multicolumn{4}{c}{Source}            && \multicolumn{4}{c}{Target}            \\ 
%               \cline{2-5} \cline{7-10} 
%               & Acc  & \multicolumn{3}{c}{Unfairness} && Acc & \multicolumn{3}{c}{Unfairness}\\
%               \cline{3-5} \cline{8-10}
% Method         &   & $V_{acc}$ & $\Delta_{acc}$ & $\Delta_{odds}$ &&    & $V_{acc}$ & $\Delta_{acc}$ & $\Delta_{odds}$ \\
% \midrule
% Base           & 90.79 &   1.73       & 2.53     & 4.88    && 74.22 & 7.01     & 4.57     & 6.62    \\
% LAFTR          & 91.00 &   1.46       & 1.68     & 3.45    && 73.74 & 4.1      & 4.73     & 8.10     \\
% LAFTR+DANN     & 90.57 &   1.63       & 2.43     & 4.53    && 73.37 & 6.46     & 4.44     & 9.91 \\
% LAFTR+FixMatch & 92.31 &   0.98       & 1.58     & 3.20    && 76.36 & 18.71    & 5.79     & 5.22    \\
% LAFTR+UDA & 93.08 &2.46 &2.37 & 5,27 &&77.47 &19.29 & 5.13 & 5.22 \\
% Ours (LAFTR+FairFixMatch) & 92.80 &   1.51       & 2.58     & 5.21    && 77.07 & 4.71     & 2.42     & 6.36  \\
% Ours (LAFTR+FairUDA) & 93.24 &2.18 & 1.59 & 3.53 && 79.65 & 11.66& 5.13 & 5.22\\
% CFair & 89.59 & 3.1 & 3.04 & 5.44 && 72.07 & 12.57 & 3.59 & 2.09\\
% CFair+FixMatch & 91.93 & 1.44 & 2.88 & 5.76 && 74.88 & 21.57 & 6.32 & 4.07 \\
% Ours(CFair+FairFixMatch) & 93.68 & 1.56 & 2.99 & 6.09 && 78.99 & 2.02 & 2.06 & 4.89 \\

% \bottomrule
% \end{tabular}\label{tab:face-vgg}
% \end{table}
